Binscatter Regressions

We introduce the package Binsreg, which implements the binscatter methods developed by Cattaneo, Crump, Farrell, and Feng (2024b,a). The package includes seven commands: binsreg, binslogit, binsprobit, binsqreg, binstest, binspwc, and binsregselect. The first four commands implement binscatter plotting, point estimation, and uncertainty quantification (confidence intervals and confidence bands) for least squares linear binscatter regression (binsreg) and for nonlinear binscatter regression (binslogit for Logit regression, binsprobit for Probit regression, and binsqreg for quantile regression). The next two commands focus on pointwise and uniform inference: binstest implements hypothesis testing procedures for parametric specifications and for nonparametric shape restrictions of the unknown regression function, while binspwc implements multi-group pairwise statistical comparisons. Finally, the command binsregselect implements data-driven number of bins selectors. The commands offer binned scatter plots, and allow for covariate adjustment, weighting, clustering, and multi-sample analysis, which is useful when studying treatment effect heterogeneity in randomized and observational studies, among many other features.

==> code/output/binsreg_out10.log.tex <==
. qui binsreg y x w, masspoints(off)
{\smallskip}


==> code/output/binsreg_out11.log.tex <==
. * note: the community-distributed package gtools needs to be installed to turn on the op
> tion usegtools()
. qui binsreg y x w, masspoints(off) usegtools(on)
Gtools package not installed.
{\smallskip}


==> code/output/binsreg_out15.log.tex <==
. tempfile file_q25 file_q75 file_reg
{\smallskip}
. preserve
{\smallskip}
. binsqreg y x, quantile(0.25) line(3 3) savedata(`file_q25')
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
{\smallskip}
Binscatter plot, quantile
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
Output file: /var/folders/0b/h0wl9g7d3s3dr9d_vm0qts9r0000gn/T//S_37285.000003.dta
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      20
                 imse, bias{\caret}2 {\VBAR}   5.501
                   imse, var. {\VBAR}   1.526
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       20
 line    {\VBAR}      3       3       23
\HLI{9}{\BOTT}\HLI{30}
{\smallskip}
. binsqreg y x, quantile(0.75) line(3 3) savedata(`file_q75')
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
{\smallskip}
Binscatter plot, quantile
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
Output file: /var/folders/0b/h0wl9g7d3s3dr9d_vm0qts9r0000gn/T//S_37285.000004.dta
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      20
                 imse, bias{\caret}2 {\VBAR}   5.501
                   imse, var. {\VBAR}   1.526
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       20
 line    {\VBAR}      3       3       23
\HLI{9}{\BOTT}\HLI{30}
{\smallskip}
. binsreg y x, line(3 3) cb(3 3) savedata(`file_reg')
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
Note: Setting at least nsims(2000) and simsgrid(50) is recommended to obtain the final res
> ults.
{\smallskip}
Binscatter plot
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
Output file: /var/folders/0b/h0wl9g7d3s3dr9d_vm0qts9r0000gn/T//S_37285.000005.dta
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      20
                 imse, bias{\caret}2 {\VBAR}   5.501
                   imse, var. {\VBAR}   1.526
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       20
 line    {\VBAR}      3       3       23
 CB      {\VBAR}      3       3       23
\HLI{9}{\BOTT}\HLI{30}
{\smallskip}
. use `file_reg', clear
{\smallskip}
. append using `file_q25' `file_q75', generate(source)
{\smallskip}
. twoway (scatter dots_fit dots_x if source==0, mcolor(navy)) ///
>        (line line_fit line_x if source==0, sort lcolor(navy)) ///
>            (rarea CB_l CB_r CB_x if source==0, sort fcolor(navy\%50) lcolor(none\%0) finte
> nsity(50)) ///
>            (line line_fit line_x if source==1, sort) ///
>            (line line_fit line_x if source==2, sort), ///
>            ytitle(Y) xtitle(X) title(Binscatter Plot) ///
>            legend(order(1 "E[Y|X]" 2 "E[Y|X]" 3 "Conf. Band for E[Y|X]" 4 "0.25 quantile
> " 5 "0.75 quantile"))
{\smallskip}
. restore
{\smallskip}


==> code/output/binsreg_out18.log.tex <==
. binslogit d x w, nolink
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
{\smallskip}
Binscatter plot, logit model
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      12
                 imse, bias{\caret}2 {\VBAR}   0.172
                   imse, var. {\VBAR}   0.208
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       12
\HLI{9}{\BOTT}\HLI{30}


==> code/output/binsreg_out19.log.tex <==
. qui binslogit d x w, logitopt(iterate(1000))
{\smallskip}


==> code/output/binsreg_out2.log.tex <==
. binsreg y x w, at(median)
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
{\smallskip}
Binscatter plot
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      21
                 imse, bias{\caret}2 {\VBAR}   5.420
                   imse, var. {\VBAR}   1.192
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       21
\HLI{9}{\BOTT}\HLI{30}


==> code/output/binsreg_out25.log.tex <==
. binstest y x w, estmethod(qreg 0.5) testmodelpoly(1)
Note: Setting at least nsims(2000) and simsgrid(50) is recommended to obtain the final res
> ults.
{\smallskip}
Hypothesis tests based on binscatter estimates
Estimation method: qreg
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      21
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
Model specification Tests:
Degree: 1     \# of smoothness constraints: 1
{\smallskip}
\HLI{19}{\TOPT}\HLI{30}
H0: mu =           {\VBAR} sup |T|           p value
\HLI{19}{\PLUS}\HLI{30}
poly. degree  1    {\VBAR}   4.420             0.000
\HLI{19}{\BOTT}\HLI{30}


==> code/output/binsreg_out26.log.tex <==
. binstest d x w, estmethod(logit) deriv(1) nbins(20) testshaper(0)
Warning: Testing procedures are valid when nbins() is much larger than the IMSE-optimal ch
> oice. Compare your choice with the IMSE-optimal one obtained by binsregselect.
Note: Setting at least nsims(2000) and simsgrid(50) is recommended to obtain the final res
> ults.
{\smallskip}
Hypothesis tests based on binscatter estimates
Estimation method: logit
Bin selection method: User-specified
Placement: User-specified
Derivative: 1
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       .
  \# of smoothness constraints {\VBAR}       .
                    \# of bins {\VBAR}      20
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
Shape Restriction Tests:
Degree: 2     \# of smoothness constraints: 2
{\smallskip}
\HLI{19}{\TOPT}\HLI{30}
H0: inf mu >=      {\VBAR} inf T             p value
\HLI{19}{\PLUS}\HLI{30}
         0         {\VBAR}  -1.417             0.958
\HLI{19}{\BOTT}\HLI{30}


==> code/output/binsreg_out34.log.tex <==
. binsregselect y x w, nbins(20) pselect(1/4)
{\smallskip}
Bin selection for binscatter estimates
Method: IMSE-optimal plug-in choice (select degree and smoothness)
Position: Quantile-spaced
{\smallskip}
\HLI{28}{\TOPT}\HLI{10}
          \# of observations {\VBAR}    1000
       \# of distince values {\VBAR}    1000
              \# of clusters {\VBAR}       .
           eff. sample size {\VBAR}    1000
\HLI{28}{\PLUS}\HLI{10}
                  \# of bins {\VBAR}      20
\HLI{28}{\BOTT}\HLI{10}
{\smallskip}
\HLI{14}{\TOPT}\HLI{8}{\TOPT}\HLI{7}{\TOPT}\HLI{7}{\TOPT}\HLI{15}{\TOPT}\HLI{14}
    method    {\VBAR}    p   {\VBAR}    s  {\VBAR}   df  {\VBAR} imse, bias{\caret}2  {\VBAR}  imse, var.  
\HLI{14}{\PLUS}\HLI{8}{\PLUS}\HLI{7}{\PLUS}\HLI{7}{\PLUS}\HLI{15}{\PLUS}\HLI{14}
   ROT-POLY   {\VBAR}    4   {\VBAR}    4  {\VBAR}   24  {\VBAR}  2984.463     {\VBAR}    5.954
   ROT-REGUL  {\VBAR}    1   {\VBAR}    1  {\VBAR}   21  {\VBAR}        .      {\VBAR}        .
   ROT-UKNOT  {\VBAR}    1   {\VBAR}    1  {\VBAR}   21  {\VBAR}        .      {\VBAR}        .
      DPI     {\VBAR}    1   {\VBAR}    1  {\VBAR}   21  {\VBAR}  468.078      {\VBAR}    1.237
   DPI-UKNOT  {\VBAR}    1   {\VBAR}    1  {\VBAR}   21  {\VBAR}        .      {\VBAR}        .
\HLI{14}{\BOTT}\HLI{8}{\BOTT}\HLI{7}{\PLUS}\HLI{7}{\BOTT}\HLI{15}{\BOTT}\HLI{14}
p: degree of polynomial. s: \# of smoothness constraints. df: degrees of freedom.


==> code/output/binsreg_out7.log.tex <==
. binsreg y x w i.t, dots(0,0) line(3,3) ci(3,3) cb(3,3) polyreg(4) ///
>                    vce(cluster id) asyvar(on) title("Binned Scatter Plot") 
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
Note: When additional covariates w are included, the polynomial fit may not always be clos
> e to the binscatter fit.
Note: Setting at least nsims(2000) and simsgrid(50) is recommended to obtain the final res
> ults.
{\smallskip}
Binscatter plot
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}     500
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      20
                 imse, bias{\caret}2 {\VBAR}   3.588
                   imse, var. {\VBAR}   0.494
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       20
 line    {\VBAR}      3       3       23
 CI      {\VBAR}      3       3       23
 CB      {\VBAR}      3       3       23
 polyreg {\VBAR}      4       NA      5
\HLI{9}{\BOTT}\HLI{30}


==> code/output/binsreg_out9.log.tex <==
. * note: the community-distributed package reghdfe needs to be installed to absorb fixed 
> effects via the option absorb()
. binsreg y x w, absorb(t) at(mean) dots(0,0) line(3,3) ci(3,3) cb(3,3) polyreg(4)
Sorting dataset on x...
Note: This step is omitted if dataset already sorted by x.
Note: When additional covariates w are included, the polynomial fit may not always be clos
> e to the binscatter fit.
Note: Setting at least nsims(2000) and simsgrid(50) is recommended to obtain the final res
> ults.
{\smallskip}
Binscatter plot
Bin selection method: IMSE-optimal plug-in choice (select \# of bins)
Placement: Quantile-spaced
Derivative: 0
{\smallskip}
\HLI{30}{\TOPT}\HLI{15}
\# of observations             {\VBAR}    1000
\# of distinct values          {\VBAR}    1000
\# of clusters                 {\VBAR}       .
\HLI{30}{\PLUS}\HLI{15}
Bin/Degree selection:         {\VBAR} 
         Degree of polynomial {\VBAR}       0
  \# of smoothness constraints {\VBAR}       0
                    \# of bins {\VBAR}      22
                 imse, bias{\caret}2 {\VBAR}   4.736
                   imse, var. {\VBAR}   0.927
\HLI{30}{\BOTT}\HLI{15}
{\smallskip}
\HLI{9}{\TOPT}\HLI{30}
         {\VBAR}      p       s       df
\HLI{9}{\PLUS}\HLI{30}
 dots    {\VBAR}      0       0       22
 line    {\VBAR}      3       3       25
 CI      {\VBAR}      3       3       25
 CB      {\VBAR}      3       3       25
 polyreg {\VBAR}      4       NA      5
\HLI{9}{\BOTT}\HLI{30}

